Byz-GentleRain: An Efficient Byzantine-tolerant Causal Consistency Protocol

Causal consistency is a widely used weak consistency model that allows high availability despite network partitions. There are plenty of research prototypes and industrial deployments of causally consistent distributed systems. However, as far as we know, none of them consider Byzantine faults, except Byz-RCM proposed by Tseng et al. Byz-RCM achieves causal consistency in the client-server model with $3f + 1$ servers where up to $f$ servers may suffer Byzantine faults, but assumes that clients are non-Byzantine. In this work, we present Byz-Gentlerain, the first causal consistency protocol which tolerates up to $f$ Byzantine servers among $3f + 1$ servers in each partition and any number of Byzantine clients. Byz-GentleRain is inspired by the stabilization mechanism of GentleRain for causal consistency. To prevent causal violations due to Byzantine faults, Byz-GentleRain relies on PBFT to reach agreement on a sequence of global stable times and updates among servers, and only updates with timestamps less than or equal to such common global stable times are visible to clients. We prove that Byz-GentleRain achieves Byz-CC, the causal consistency variant in the presence of Byzantine faults. We evaluate Byz-GentleRain on Aliyun. The preliminary results show that Byz-GentleRain is efficient on typical workloads.

==> algs/byz.tex <==
% byz.tex

\begin{algorithm}[t]
  \label{Byzantine_logic_server}
  \IncMargin{1em}
  \DontPrintSemicolon
  \caption{Broadcast request}

  \s(){} \;
  \proc(initialization:){
  	$\rm prepared\_num$ $\leftarrow$ 0 \;
  	$\rm commit\_num$ $\leftarrow$ 0 \;
  	$\rm finish\_num$ $\leftarrow$ 0 \;
  	$\rm local_{msg}$ $\leftarrow$ initial \;
  }

  \upon({\receive $({\rm REQUEST}, op_{msg})$ from client $c$})
  {
  	check digital signature and digital encryption \;
  	$\rm prepared\_num$++ \;
  	$\rm local_{msg}$ $\leftarrow$ $\rm op_{msg}$ \;
  	\send $({\rm PREPARED}, op_{msg})$ to all replicas \;
  }

  \upon({\receive $({\rm PREPARED}, op_{msg})$ from  $s_j$})
  {
  	check digital signature and digital encryption \;
  	check whether $op_{msg}$ and $\rm local\_msg$ are the same \;
  	\If{check(msg)}{${\rm prepared\_num}$++} \;
  	\If{$\rm prepared\_num$ $\geq$ $3f+1$} {
  		$\rm commit\_num$++ \;
  		\send $( {\rm COMMIT} , op_{msg} )$ to all replicas \;
  	}
  }

  \upon({\receive $({\rm COMMIT}, op_{msg})$ from  $s_j$})
  {
  	check digital signature and digital encryption \;
  	check whether $op_{msg}$ and $\rm local\_msg$ are the same \;
  	\If{check(msg)}{$\rm commit\_num$++} \;
  	\If{$\rm commit\_num$ $\geq$ $3f+1$}{
  		$\rm ACK$ $\leftarrow$ ${\rm deal\_request}$ $(op_{msg})$ \;
  		\send $\rm ACK$ to client $c$ \;
  		\send $( {\rm FINISH} , op_{msg} )$ to all replicas \;
  	}
  }

  \upon({\receive $({\rm FINISH}, op_{msg})$ from  $s_j$})
  {
  	check digital signature and digital encryption \;
  	\If{$\rm local_{msg} = initial$}{
  		$\rm local_{msg}$ $\leftarrow$ $\rm op_{msg}$ \;
  	}
  	check whether $op_{msg}$ and $\rm local\_msg$ are the same \;
  	\If{check(msg)}{$\rm finish\_num$++} \;
  	\If{$\rm finish\_num$ $\geq$ $3f+1$}{
  		$\rm ACK$ $\leftarrow$ ${\rm deal\_request}$ $(op_{msg})$ \;
  		\send $\rm ACK$ to client $c$ \;
  		\send $( {\rm FINISH} , op_{msg} )$ to all replicas \;
  	}
  }
\end{algorithm}

==> algs/cgst-4f+1.tex <==
% cgst-4f+1.tex

\begin{algorithm}[t]
  \caption{Update $\cgst$ at replica $\replica{\pvar}_{\dvar}$}
  \label{alg:cgst-4f+1}
  \begin{algorithmic}[1]
	% \Procedure{\newupdates}{$\cgstvar$}
	%   \State $\send \Call{\textsc{GET\_UPDATES}}{\cgstvar} \sendto \Call{\replicas}{m}$

	%   \hStatex
	%   \State \wait\receive $\Call{\textsc{GET\_UPDATES\_ACK}}{\cgstvar, \storevar^m_i}$ from $3f+1$ replicas
	%   \State $\storevar^m \gets \bigcup_{i} \storevar^m_i$ $\forall i$
	%   \State \Return $\storevar^m$
	% \EndProcedure
	\Upon[$\Call{\newview}{v}$]
		\State $\currview \gets v$
		\State $\voted \gets \false$
		\State $\sf prepared\_value \gets \{\cgstvar, \storevar^m\}$
		\State $\send \tuple{\Call{\newleader}{\currview, \preparedview, \preparedstore, cert}}^{m}_{d} \sendto \replica{m}{v}$
	\EndUpon

	\Statex
	\WhenReceive[$\set{\tuple{\Call{\newleader}{v, \viewvar_i, val_i, cert_i}}^{m}_{i}
	  \mid p^m_i \in Q} = C$ {\bf from a quorum $Q$}]
      %pre: curr view = v ^ pi = leader(v) ^ (8m 2 C. ValidNewLeader(m));
      \State \pre $\currview = \mathit{v} \land p^m_d = leader(\mathit{v})$\\
      \hspace{20pt} $\land (\forall m \in C.\; ValidNewLeader(m))$

	  \hStatex
	  \If{$\exists j.\; \viewvar_j = \max\set{\viewvar_k \mid \replica{m}{k} \in Q} \neq \bot$}
	    \State	$\send \tuple{\Call{\propose}{v, cgst, \storevar^m, C}}^m_d \sendto \replicas(m)$
	  \Else
	  	\State $\send \Call{\collect}{\cgstvar} \sendto \red{\Call{\replicas}{m}}$
	  	\State \wait\receive $\Call{\collectack}{\cgstvar, \storevar_{i}}$ \\
	  	  \hspace{35pt} {\bf \red{from a set $Q$ of $3f+1$ replicas}, for $i \in Q$}
	  	\State $\storevar \gets \bigcup\limits_{i \in Q} \storevar_i$
	  	\State $\send \tuple{\Call{\propose}{v, \cgst, \storevar, C}}^m_d \sendto \replicas(m)$
	  \EndIf
	\EndWhenReceive

	\Statex
	\WhenReceive[$\tuple{\Call{\propose}{v,cgst, \storevar, C}}^m_i = \mvar$]
	  \label{line:procedure-propose}
	  \State \pre $\red{\currview = v} \land \safe(\mvar) \land \voted = \false $
	    \label{line:prepare-pre}

	  \hStatex
	  \State $\sf cur\_cgst \gets \cgstvar$
	  \State $\sf cur\_\store \gets \storevar$
	  \State $\voted \gets \true$
	  \hStatex
	  \If{\red{$\store \setminus \storevar = \emptyset$} $\land$ \red{$C(\storevar) = true$}}
	    \label{line:prepare-check-dt}
        \State $\send \tuple{\Call{\prepared}{v, \green{\hash(\cgstvar, \storevar)}, \trust}}^{m}_{d}$ \\
		  \hspace{30pt} $\sendto \replicas(m)$
	      \label{line:propose-send-prepared-trust}
   	  \Else
    	\State $\send \tuple{\Call{\prepared}{v, \green{\hash(\cgstvar, \storevar)}, \doubt}}^{m}_{d}$ \\
		  \hspace{30pt} $\sendto \replicas(m)$
	      \label{line:propose-send-prepared-doubt}
       \EndIf
  	\EndWhenReceive

	\Statex
  	\WhenReceive[$\set{\tuple{\Call{\prepared}{v, \cgstvar, \storevar^m, h, \_}}^{m}_{i}
	  \mid i \in Q} = \mvar$
	  {\bf from a set $Q$ of $3f+1$ replicas such that} \\
	  \hspace{5pt} $|\set{\prepared(\_, \_, \trust)} \in \mvar| \ge 2f+1$]
	  \label{line:procedure-prepared}
	  \State \pre $\sf \currview = v \land hash(\cgstvar, \storevar^m) = h \land \voted = \true$
	    \label{line:prepared-pre}
	  \State $\preparedview \gets \currview$
	  \State $\sf pre\_cgst \gets \sf cur\_cgst$
	  \State $\sf pre\_\store^m \gets \storevar^m$
	  \State $\sf cert \gets C$
	  \hStatex
	  \State $\red{\lockedcgst} \gets \currcgst$
	    \label{line:prepared-lockedcgst}
	  \State $\red{\preparedstore} \gets \storevar^m$
	    \label{line:prepared-preparedstore}
	  \State $\send \tuple{\Call{\commit}{v, \cgstvar, \storevar^m,
	    \hash(\cgstvar, \storevar^m)}}^{m}_{d}$ \\
	    \hspace{20pt} $\sendto \replicas(m)$
		\label{line:prepared-send-commit}
  	\EndWhenReceive

	\Statex
	  \WhenReceive[$\set{\tuple{\Call{\commit}{v, \cgstvar, \storevar^m, h}}^{m}_{i} \mid i \in Q} = M$
		{\bf from a set $Q$ of $3f+1$ replicas}]
	    \label{line:procedure-commit}
	  \State \pre $\currview = \preparedview = v \land\;$ \\
	    \hspace{32pt} \green{$\hash(\cgstvar, \storevar^m) = h$}
	    \label{line:commit-pre}

	  \hStatex
  	  \State \red{decide$(\cgstvar, \storevar^m)$}
		\label{line:commit-store}
	  \EndWhenReceive

	\Statex
	\WhenReceive[$\Call{\collect}{\cgstvar}$]
	  \State \red{$\currcgst \gets \cgstvar$; status???}
	  \State $\storevar \gets \set{\tuple{\_, \utvar, \_} \in \store \mid \utvar \le \red{\cgstvar}}$
	  \State $\send \tuple{\Call{\collectack}{\cgstvar, \storevar}}^{j}_{i} \sendto \replica{j}{i}$
	\EndWhenReceive
  \end{algorithmic}
\end{algorithm}

==> algs/cgst-backup.tex <==
% cgst-backup.tex

\begin{algorithm}[t]
  \caption{Update $\cgst$ at replica $\replica{m}{d}$}
  \label{alg:cgst}
  \begin{algorithmic}[1]
  	\WhenReceive[$\langle\Call{\newcgst}{\cgstvar}\rangle^m_i = m $]
	    \label{line:procedure-updatecgs}
		\Comment{\red{Signature???}}
	  \State \pre $\cgstvar \le \lst$ $\wedge$ $\sf safe(m)$
	    \Comment{\red{when $\cgstvar > \lst$???}}
	    \label{line:cgst-cgstvar-le-lst}
  	  \State \red{stop accepting updates $\le \cgstvar$??? implementation???}
		\label{line:cgst-stop}
  	  \State $\storevar \gets \set{\tuple{\_, \utvar, \_} \mid \utvar \le \red{\cgstvar}}$
		\label{line:cgst-storevar}
  	  \State $\send \Call{\newcgstack}{\cgstvar, \storevar} \sendto \replica{m}{i}$
		\label{line:cgst-send-newcgstack}
  	\EndWhenReceive

	\Statex
  	\WhenReceive[$\Call{\newcgstack}{\cgstvar_{i}, \storevar_{i}}$ \\
	    \hspace{5pt} {\bf from} a set $Q$ of $3f + 1$ replicas,
		  ranged over by $i \in Q$]
		\label{line:procedure-newcgstack}
  	  \State pack all these $versions$ in a vector $syn\_versions$
  	  \State $\send \Call{syn\_cgst}{\cgstvar, syn\_versions}$ to all replicas
  	\EndWhenReceive

	\Statex
  	\WhenReceive[$\Call{sync\_cgst}{\cgstvar, sync\_versions} \from \replica{m}{r}$]
	  \label{line:procedure-synccgst}
	  \Comment{\red{integrated into \newcgstack???}}
  	\If{some updates lost in $syn\_versions$}
  	  \State $\send \Call{\prepare}{\cgst, sync\_versions, \doubt}$ to all replicas
		\label{line:synccgst-send-prepare-doubt}
  	\Else
  	  \State $\send \Call{\prepare}{\cgst, sync\_versions, \trust}$ to all replicas
		\label{line:synccgst-send-prepare-trust}
  	\EndIf
  	\EndWhenReceive

	\Statex
  	\WhenReceive[$\Call{\prepare}{\cgstvar_{i}, versions_{i}, \_}$ \\
	  \hspace{5pt} {\bf from} a set $Q$ of $3f+1$ replicas, ranged over by $i \in Q$, \\
	  \hspace{10pt} such that \red{$|\set{\prepare(\_, \_, \trust)} \in Q| \ge 2f+1$}]
  	  \State $\send \Call{\commit}{\cgstvar, syn\_versions}$ to all replicas
  	\EndWhenReceive

	\Statex
  	\WhenReceive[$\Call{\commit}{\cgstvar, syn\_versions}$ \\
	  \hspace{5pt} {\bf from} a set $Q$ of $2f+1$ replicas]
  	  \State store $(\cgstvar, syn\_versions)$
  	  \State $\cgst \gets \cgstvar$
  	\EndWhenReceive

	\Statex
  	\Upon[timeout and has not collocted enough msg]
  	  \State $\send \Call{\withdraw}{\cgstvar, syn\_versions}$ to all replicas
  	\EndUpon

	\Statex
  	\WhenReceive[$f+1$ $\Call{\withdraw}{\cgstvar, syn\_versions}$ ]
  	  \State delete $(\cgstvar, syn\_versions)$
  	\EndWhenReceive
    \end{algorithmic}
\end{algorithm}

==> algs/headbeat-extension.tex <==
% cgst-backup.tex

\begin{algorithm}[t]
  \caption{Update $\cgst$ at replica $\replica{m}{d}$}
  \label{alg:cgst}
  \begin{algorithmic}[1]\WhenReceive[$\tuple{\Call{\propose}{v,x,C}}^{m}_{j} = m$]
	\label{line:procedure-newcgst}
	\State \pre $x.\cgstvar \le \lst
	  \land v = \currview \land voted = FALSE \land SafeProposal(m)$
	  \label{line:newcgst-pre}
	\hStatex
	  \State \red{stop accepting updates $\le \cgstvar$; status???}
	  \label{line:cgst-stop}
	  \State $\storevar \gets \set{\tuple{\_, \utvar, \_} \in \store
		\mid \utvar \le \red{\cgstvar}}$
	  \label{line:cgst-storevar}
	  \State $\send \tuple{\Call{\newcgstack}{\cgstvar, \storevar}}^{j}_{i} \sendto \replica{j}{i}$
	  \label{line:cgst-send-newcgstack}
	\EndWhenReceive

  \Statex
	\WhenReceive
	[$\set{\tuple{\Call{\newcgstack}{\cgstvar, \storevar^{j}_{i}}}^j_i \mid i \in Q} = \mvar$
	{\bf from a set $Q$ of $3f + 1$ replicas}, {\bf for $1 \le j \le P$}]
	\label{line:procedure-newcgstack}
	\State \red{\pre $\cgstvar \le \lst \land \green{\safe(\mvar)}
	  \land \neg \valid(\cgstvar)$}
	  \label{line:newcgstack-pre}

	\hStatex
	\State $\storevar^{j} \gets \bigcup\limits_{i \in Q} \storevar^{j}_{i}$,
	  {\bf for} $1 \le j \le P$
	  \label{line:newcgstack-storevar}
	\State $\send \tuple{\Call{\propose}{\cgstvar, \storevar^{j}}}^{m}_{d}$
	  {\bf to} $\replicas(j)$, {\bf for} $1 \le j \le P$
	  \label{line:newcgstack-send-propose}
	\EndWhenReceive
	\Statex
	\Upon[timeout and has not collocted enough msg]
	  \State $\send \tuple{\Call{\withdraw}{\cgstvar}}$ $\sendto$ all replicas
	\EndUpon

  \Statex
	\WhenReceive[$f+1$ $\tuple{\Call{\withdraw}{\cgstvar}}$ ]
	  \State delete $\tuple{(\cgstvar, \storevar^m)}$
	\EndWhenReceive
  \end{algorithmic}
    \end{algorithmic}
\end{algorithm}

==> sections/discussion.tex <==
% discussion.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discussions} \label{ss:discussions}

%%%%%%%%%%%%%%%%%%%%
\subsubsection{Optimization} \label{sss:optimization}

If the physical clock of a client is much later
than the physical clocks in other processes,
its updates may be refused and it has to reset the physical clock.
Replicas will refuse these updates
because byzantine clients may update a value
with an old timestamp to break the causality.
In this case, a correct client needs to reset its physical clock
and update the value again.
Since the physical clock increases all time
and the $FGST$ that replicas maintain increases by update events,
this case seldom take place in a correct client,
unless its physical clock is broken.
%%%%%%%%%%%%%%%%%%%%
\subsubsection{Liveness} \label{sss:liveness}

Let $ml$ denote the maximum network delay between the system,
$lt_r$ denote the lower bound of the physical time on replicas,
and $lt_c$ denote the lower bound of the physical time on clients.
If $lt_c - ml > lt_r$,
then all the updates sent by a correct client will be valid,
which means correct clients will not propose an update
with a timestamp older than $FGST$.

Ideally, all the processes share the same physical clock
and the network latency tends to be zero.
In this case $lt_c - ml = lt_r$,
so the property ensures that all the updates from correct clients will be valid.
Now let us relax the requirement for clock synchronization and network latency.
If a new update form $c$ has a too old timestamp $t_c$,
then its physical clock is too slow or the network latency $l_{cr}$ is too long,
which means $t_c - l_{cr}$ is too small.
Though we cannot control $t_c$ and $l_{cr}$,
we can set a reasonable lower bound.
Here we choose $lt_r$(the lower bound of current physical time on replicas),
because clients with a correct physical clock will finally satisfy the inequality.
If the physical clock of client $c$ works correctly,
then $t_c - lt_r > k$, where $k$ is a constant.
By adding an offset to the physical clock,
it will finally satisfy that $t_c - lt_r > l_{cr}$,
and then the client can keep proposing its update.
If the whole system satisfying $lt_c - ml > lt_r$,
then all the updates sent by a correct client
will be valid by the third property 'reasonable'.
Otherwise, a client will be told to reset its physical time and retry its update.
By resetting physical clock and giving an offset to $t_c$,
it will finally propose updates successfully.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/implementation.tex <==
\section{Evaluation}

We evaluate Byz-GentleRain in terms of local latencies, through\_put, and remote update visibility latency, 
by varying the workloadss. 
We compare Byz-GentleRain to Byz-RCM.

\subsection{Implementation and Setup}

We implement Byz-GentleRain in Java and use Google’s Protocol Buffers for message serialization. 
We also implement Byz-RCM in the same code base for performance comparison. 
The data store is a key-value store. The data set used
in the experiments contains one thousand key-value pairs, 
with the key size being eight bytes and the value
size 64 bytes. The key-value store keeps all key-value pairs
in main memory. 
A key points to a linked list that contains
different versions of the same item. 
A PUT operation inserts a new version to the version 
chain of the updated item and
adds a record to the operation log.
We use Date class to keep physical clocks synchronized. We
configure it to change clock frequency, so that our physical
clocks always move forward, a requirement for correctness
in Byz-GentleRain.

We run all experiments on Alibaba Cloud
instances running Ubuntu 12.04. 
Each server has $x$ virtual
CPU cores, $x$ GB memory, and $x$ 16GB SSD storage.
We replicate each dataitem at three replicas.

\subsection{Throughput}

\subsection{Update Visibility Latency}

\begin{figure}
    \includegraphics[width=\columnwidth]{figs/latency.png}
    \includegraphics[width=\columnwidth]{figs/get_latency.png}
    \includegraphics[width=\columnwidth]{figs/FGST_update.png}
\end{figure}

==> sections/sign-checking.tex <==
% sign-checking.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sign checking} \label{sign checking}

%%%%%%%%%%%%%%%%%%%%
\begin{definition}
    Safe_
\end{definition}
%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/performance.tex <==
% performance.tex

\begin{table}[t]
  \centering
  \caption{\red{??? units???}}
  \begin{tabular}{c|c|c}
    \hline
  	    & \put & \get \\
  	\hline
    \byzrcm & 73.8 & 67.8 \\
    \byzgentlerain & 64.9 & 107.8 \\
    \hline
  \end{tabular}
\end{table}
